Techni-Composite Higgs models with (a)symmetric dark matter candidates

We propose a novel class of composite models that feature both a technicolor and a composite Higgs vacuum limit, resulting in an asymmetric dark matter candidate. These Techni-Composite Higgs models are based on an extended left-right electroweak symmetry with a pseudo-Nambu Goldstone boson Higgs and stable dark matter candidates charged under a global $\mathrm{U}(1)_X$ symmetry, connected to the baryon asymmetry at high temperatures via the $SU(2)_{\rm R}$ sphaleron. We consider, as explicit examples, four-dimensional gauge theories with fermions charged under a new confining gauge group $G_{\rm HC} $.

==> Letter arXiv version/SupplementaryMaterial_included.tex <==
%%\documentclass[aps,prd,amsmath,amssymb,superscriptaddress,altaffillsymbol, preprintnumbers,preprint,nofootinbib,a4paper]{revtex4}
%\documentclass[amsmath,amssymb,preprintnumbers,nofootinbib,prd,a4paper,onecolumn]{revtex4-1}
%\pdfoutput=1
%
%\usepackage{amsthm}
%\usepackage{amsmath}
%\usepackage{graphicx}
%\usepackage{bbold}
%\usepackage{color}
%\usepackage{subfigure}
%\usepackage{multirow}
%\usepackage{graphicx,bm}
%\usepackage{physics}
%
%\usepackage{dcolumn}% Align table columns on decimal point
%\usepackage{bm}% bold math
%\usepackage{slashed}
%\usepackage{epsfig}
%\usepackage{hyperref}
%\usepackage{verbatim}
%%\usepackage{unicode-math}
%
%
%\usepackage[utf8]{inputenc}
%\usepackage[T1]{fontenc}
%\usepackage[normalem]{ulem}
%
%\newcommand{\beq}{\begin{eqnarray}}
%\newcommand{\eeq}{\end{eqnarray}}
%\newcommand{\nn}{~\nonumber \\}
%\newcommand{\p}{{\cal P}\exp}
%\newcommand{\texp}{{\cal T}\exp}
%\newcommand{\ssh}{\gam ma\cdot}
%\newcommand{\im}{{\rm Im}}	
%\newcommand{\bmp}{\noindent\begin{minipage}{16cm}}
%\newcommand{\emp}{\end{minipage}\vskip 7mm} % 7mm untightened
%\newcommand{\unsplit}{\check}
%\newcommand{\system}{\hat}
%\newcommand{\kernel}{\bar}
%\newcommand{\wt}{\widetilde}
%\newcommand{\sigmaf}{\sigma\hspace{-1mm}:\hspace{-1mm}F}
%\newcommand{\erer}{\, \bar e_R e^C_R}
%\newcommand{\llS}{\,\bar l_L  i\tau_2  l^C_L}
%\newcommand{\llT}{\,\bar l_L  T_L  l^C_L}
%\newcommand{\llTc}{\,\bar l_L \left( i \tau_2 \, T^{\dagger}_L \, i \tau_2 \right)  l^C_L}
%\newcommand{\E}{\mathcal{E}}
%
%\newcommand{\MeV}{\mbox{ ${\mathrm{MeV}}$}}
%\newcommand{\GeV}{\mbox{ ${\mathrm{GeV}}$}}
%\newcommand{\TeV}{\mbox{ ${\mathrm{TeV}}$}}
%\newcommand{\ifb}{\mbox{ ${\mathrm{fb^{-1}}}$}}
%\newcommand{\uni}{\mbox{ ${\bf 1}_{2\times 2}$ }}
%%\newcommand{\Tr}{\mbox{Tr}\;}
%\newcommand{\be}{\begin{eqnarray}}
%\newcommand{\ee}{\end{eqnarray}}
%\newcommand{\gt}{\widetilde{g}}
%\newcommand{\SU}{\mbox{SU}}
%\newcommand{\SO}{\mbox{SO}}
%\newcommand{\SP}{\mbox{Sp}}
%\newcommand{\UU}{\mbox{U}}
%
%\newcommand{\st}{s_\theta}
%\newcommand{\ct}{c_\theta}
%\newcommand{\stt}{s_{2\theta}}
%\newcommand{\ctt}{c_{2\theta}}
%
%\newcommand{\com}[1]{{\color{red}{ #1 }}}
%\newcommand{\add}[1]{{\color{blue}{ #1 }}}
%
%\def\eq#1{{eq.~(\ref{#1})}}
%\def\eqs#1#2{{eqs.~(\ref{#1})--(\ref{#2})}}
%\def\fig#1{{fig.~(\ref{#1})}}
%\def\sec#1{{sec.~(\ref{#1})}}
%\def\tab#1{{tab.~(\ref{#1})}}
%\def\CM{{\cal M}}
%
%% -----------------------------------------------------------------------------
%% Young tableaux
%% -----------------------------------------------------------------------------
%
%% draw box with width #1pt and line thickness #2pt
%\newcommand{\drawsquare}[2]{\hbox{%
%	\rule{#2pt}{#1pt}\hskip-#2pt%  left vertical
%	\rule{#1pt}{#2pt}\hskip-#1pt%  lower horizontal
%	\rule[#1pt]{#1pt}{#2pt}}\rule[#1pt]{#2pt}{#2pt}\hskip-#2pt%  upper horizontal
%\rule{#2pt}{#1pt}}% right vertical
%
%\newcommand{\Yfund}{\raisebox{-.5pt}{\drawsquare{6.5}{0.4}}}%  fund
%\newcommand{\Ysymm}{\raisebox{-.5pt}{\drawsquare{6.5}{0.4}}\hskip-0.4pt%
%\raisebox{-.5pt}{\drawsquare{6.5}{0.4}}}%  symmetric second rank
%\newcommand{\Ythrees}{\raisebox{-.5pt}{\drawsquare{6.5}{0.4}}\hskip-0.4pt%
%\raisebox{-.5pt}{\drawsquare{6.5}{0.4}}\hskip-0.4pt%
%\raisebox{-.5pt}{\drawsquare{6.5}{0.4}}}%  symmetric third rank
%\newcommand{\Yfours}{\raisebox{-.5pt}{\drawsquare{6.5}{0.4}}\hskip-0.4pt%
%\raisebox{-.5pt}{\drawsquare{6.5}{0.4}}\hskip-0.4pt%
%\raisebox{-.5pt}{\drawsquare{6.5}{0.4}}\hskip-0.4pt%
%\raisebox{-.5pt}{\drawsquare{6.5}{0.4}}}%  symmetric fourth rank
%\newcommand{\Yasymm}{\raisebox{-3.5pt}{\drawsquare{6.5}{0.4}}\hskip-6.9pt%
%\raisebox{3pt}{\drawsquare{6.5}{0.4}}}%  antisymmetric second rank
%\newcommand{\Ythreea}{\raisebox{-3.5pt}{\drawsquare{6.5}{0.4}}\hskip-6.9pt%
%\raisebox{3pt}{\drawsquare{6.5}{0.4}}\hskip-6.9pt
%\raisebox{9.5pt}{\drawsquare{6.5}{0.4}}}
%\newcommand{\Yfoura}{\raisebox{-3.5pt}{\drawsquare{6.5}{0.4}}\hskip-6.9pt%
%\raisebox{3pt}{\drawsquare{6.5}{0.4}}\hskip-6.9pt
%\raisebox{9.5pt}{\drawsquare{6.5}{0.4}}\hskip-6.9pt
%\raisebox{16pt}{\drawsquare{6.5}{0.4}}}
%\newcommand{\Yadjoint}{\raisebox{-3.5pt}{\drawsquare{6.5}{0.4}}\hskip-6.9pt%
%\raisebox{3pt}{\drawsquare{6.5}{0.4}}\hskip-0.4pt
%\raisebox{3pt}{\drawsquare{6.5}{0.4}}}%  SU(3) adjoint
%\newcommand{\Ysquare}{\raisebox{-3.5pt}{\drawsquare{6.5}{0.4}}\hskip-0.4pt%
%\raisebox{-3.5pt}{\drawsquare{6.5}{0.4}}\hskip-13.4pt%
%\raisebox{3pt}{\drawsquare{6.5}{0.4}}\hskip-0.4pt%
%\raisebox{3pt}{\drawsquare{6.5}{0.4}}}%  4 boxes in a square
%\newcommand{\Yflavor}{\Yfund + \overline{\Yfund}} % box anti-box pair
%\newcommand{\Yoneoone}{\raisebox{-3.5pt}{\drawsquare{6.5}{0.4}}\hskip-6.9pt%
%\raisebox{3pt}{\drawsquare{6.5}{0.4}}\hskip-6.9pt%
%\raisebox{9.5pt}{\drawsquare{6.5}{0.4}}\hskip-0.4pt%
%\raisebox{9.5pt}{\drawsquare{6.5}{0.4}}}%



%\begin{document}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\title{Techni-Composite Higgs models 
%	%of extended electroweak sectors 
%	with (a)symmetric dark matter candidates:\\
%	Supplementary Material}
%%%%%%%%%%
%
%\author{Giacomo {\sc Cacciapaglia}}
%\email{g.cacciapaglia@ipnl.in2p3.fr}
%\affiliation{Institut de Physique des 2 Infinis (IP2I),
%	CNRS/IN2P3, UMR5822, 69622 Villeurbanne, France}
%\affiliation{Universit\' e de Lyon, Universit\' e Claude Bernard Lyon 1, 69001 Lyon, France}
%
%\author{Mads T. {\sc Frandsen}}
%\email{frandsen@cp3.sdu.dk}
%\affiliation{CP$^3$-Origins, University of Southern Denmark, Campusvej 55, DK-5230 Odense M, Denmark}
%\author{Wei-Chih {\sc Huang}}
%\email{huang@cp3.sdu.dk}
%\affiliation{CP$^3$-Origins, University of Southern Denmark, Campusvej 55, DK-5230 Odense M, Denmark}
%\author{Martin {\sc Rosenlyst}}
%\email{rosenlyst@cp3.sdu.dk}
%\affiliation{CP$^3$-Origins, University of Southern Denmark, Campusvej 55, DK-5230 Odense M, Denmark}
%
%\author{Philip {\sc Sørensen}}
%\email{philip.soerensen@desy.de}
%%\affiliation{}
%\affiliation{DESY, Notkestra{\ss}e 85, 22607 Hamburg, Germany}
%\affiliation{II. Institute of Theoretical Physics, Universit\"{a}t  Hamburg, 22761 Hamburg, Germany}

%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\bigskip
%{\bf Supplementary Material:} 
%\maketitle

\renewcommand{\thesubsection}{S\arabic{subsection}}
\setcounter{section}{0}
\renewcommand{\thefigure}{F\arabic{figure}}
\setcounter{figure}{0}
\renewcommand{\thetable}{T\arabic{table}}
\setcounter{table}{0}
\renewcommand{\theequation}{E\arabic{equation}}
\setcounter{equation}{0}


\begin{center}
	\Large 
\textbf{Supplementary material}
\end{center}



\section{Effective Lagrangian and vacuum alignment}
We consider the scenario with $ \mathcal{R}_R$ real and $\mathcal{R}_L$ pseudoreal of $G_{\rm HC}$, which applies to the model studied in the main text. To describe the general vacuum alignment in the effective Lagrangian of this scenario, we identify an $ \SU(2)_{\rm L}\times \UU(1)_{\rm Y'} $ subgroup in $ \SU(4)_{L} $ by the generators \begin{equation}\begin{aligned}
T_{L{\rm L}}^i &= \begin{pmatrix} \sigma_i & 0 \\  0  & 0 \end{pmatrix}, \quad T_{L{\rm Y'}}^3 = \begin{pmatrix} 0 & 0 \\  0  & -\sigma_3^T \end{pmatrix},
\end{aligned} \end{equation} and an $ \SU(2)_{\rm R}\times \UU(1)_{\rm Y'} $ subgroup in $ \SU(4)_{R} $ by the generators\begin{equation}\begin{aligned}
T_{R{\rm R}}^i &= \begin{pmatrix} \sigma_i & 0 \\  0  & 0 \end{pmatrix}, \quad T_{R{\rm Y'}}^3 = \begin{pmatrix} 0 & 0 \\  0  & -\sigma_3^T \end{pmatrix},
\end{aligned} \end{equation} where $ \sigma_i $ are the Pauli matrices with $ i=1,2,3 $. Note that the $ \rm Y' $-charge generator is identified as ${\rm Y'} \equiv T^3_{L{\rm Y'}} + T^3_{R{\rm Y'}}$, while the standard hypercharge is given by ${\rm Y} \equiv T_{L{\rm  Y'}}^3 + T_{R{\rm R}}^3 +T_{R{\rm Y'}}^3$ after the breaking of $\SU(2)_{\rm R}$. Furthermore, $T_{L{\rm Y'}}^3$ and $T_{R{\rm Y'}}^3$ are part of global $\SU(2)$ symmetries that define a custodial symmetry in both cosets \cite{Georgi:1984af}. This is required in the $L$-coset to reproduce the correct $Z$/$W$ mass ratio.

The alignment between the extended EW subgroup $ \SU(2)_{\rm L}\times \SU(2)_{\rm R}\times \UU(1)_{\rm Y'} $ and the stability group $ \SP(4)_{L}\times \SO(4)_{R} $ can then be conveniently parameterized by one misalignment angle, $ \theta_{L} $. To do so, we  identify the vacua that leave the $ \SU(2)_{\rm L}\times \UU(1)_{\rm Y} $ symmetry intact, $ E_{L}^\pm $, and the one breaking $ \SU(2)_{\rm L}\times \UU(1)_{\rm Y} $ to $ \UU(1)_{\rm EM} $, $ E_{L}^B $. In the $R$-coset, there is no vacuum that preserves $ \SU(2)_{\rm R}\times \UU(1)_{\rm Y'}$, hence we define the one breaking the gauge group to $\UU(1)_{\rm Y}$, $ E_{R}^B$. They are given in term of two-index $\SU(4)$ matrices as:
\begin{equation}\begin{aligned}
E_L^\pm &= \begin{pmatrix} i\sigma_2 & 0 \\  0  & \pm i\sigma_2  \end{pmatrix}, \quad E_L^B = \begin{pmatrix} 0 & \mathbb{1}_2 \\ - \mathbb{1}_2  & 0 \end{pmatrix},   \\ E_R^B &= \begin{pmatrix} 0 & \mathbb{1}_2 \\  \mathbb{1}_2  & 0 \end{pmatrix}.
\end{aligned} \end{equation} 
Either choice of $ E_L^\pm $ is equivalent \cite{Galloway:2010bp}, and in this letter we have chosen $ E_L^- $. The true $ \SU(4)_{L} $ vacuum can be written as a linear combination of the above vacua, $ E_{L}(\theta_L) = c_{\theta_{L}}E_{L}^- + s_{\theta_{L}}E_{L}^B $ (a CH vacuum), while the vacuum of the $ \mathbb{S}_R $ sector is $ E_{R}\equiv E_R^B $ (a TC-like vacuum). We use the short-hand notations $ s_x\equiv \sin x $, $ c_x\equiv \cos x $ and $ t_x\equiv \tan x $ throughout.

The Goldstone excitations around the vacuum are then parameterized by \begin{align}
\begin{split}
\Sigma_L(x) &= \exp\left[ 2\sqrt{2}\, i \left( \frac{\Pi_L(x) }{f_L}+\frac{\Pi_\Theta(x)}{f_\Theta}\right)\right] E_L(\theta_L), \\
\Sigma_R(x) &= \exp\left[ 2\sqrt{2}\, i \left( \frac{\Pi_R(x) }{f_R}-\frac{ \Pi_\Theta(x)}{f_\Theta}\right)\right] E_R, 
\end{split}
\end{align} 
where the pion matrices $\Pi_x$ are defined as
\begin{align}
\begin{split}
&\Pi_{L}(x)=\sum^5_{i=1} \Pi_L^i X_L^i  \in G_{L}/H_{L}, \\&
\Pi_{R}(x)=\sum^9_{a=1} \Pi_R^a X_R^a  \in G_{R}/H_{R}, \\&
\Pi_\Theta(x)=\Theta(x)\ \frac{\mathbb{1}_4}{4} \in \UU(1)_\Theta/\varnothing\,.
\end{split}
\end{align} 
The last one encodes the diagonal pNGB state $ \Theta $ associated with the broken global symmetry group $ \UU(1)_\Theta $, acting on the two fermion representations and having no gauge anomaly with the HC group. 
The matrices $ X_L^i $ are the $ \theta_L $-dependent  broken generators of $ \SU(4)_{L} $, while $X_R^a$ are the broken generators of $ \SU(4)_{R} $. While in general the decay constants are different, for simplicity from now on we will assume $ f\equiv f_{L,R}=f_\Theta $.



In the $ \mathbb{S}_L $ sector, we identify the would-be Higgs boson as $ h\equiv \Pi_L^4 \sim c_{\theta_L}(\overline{U}U+\overline{D}D)+s_{\theta_L}{\rm Re}\ U^T\mathcal{C}D $ and the singlet pNGB as $ \eta\equiv  \Pi_L^5 \sim {\rm Im}\ U^T\mathcal{C}D  $, while the remaining three $ \Pi_L^{1,2,3} $ are exact Goldstones eaten by the massive $ W^\pm $ and $ Z $. In the $ \mathbb{S}_R $ sector, we identify the complex isotriplet scalars, \begin{align}
\begin{split}
&\Pi_{CS}^0\equiv \frac{\Pi_R^8+i\Pi_R^9}{\sqrt{2}}\sim C^T \mathcal{C}S, \\ 
&\Pi_{CC}^+\equiv \frac{\Pi_R^4+i\Pi_R^5+\Pi_R^6+i\Pi_R^7}{2}\sim C^T \mathcal{C}C, \\
&\Pi_{SS}^-\equiv \frac{\Pi_R^4+i\Pi_R^5-\Pi_R^6-i\Pi_R^7}{2}\sim S^T \mathcal{C}S, 
\end{split}
\end{align} where $ \Pi_{CS,\overline{CS}}^0 $ is identified as the DM candidate. The remaining three, $ \Pi_R^{1,2,3} $, are exact Goldstones eaten by the massive $ W_{\rm R}^\pm $ and $ Z_{\rm R} $. Note that, following Ref.~\cite{Ryttov:2008xe}, we have used Dirac spinors to indicate the hyperfermions, combining the $\SU(2)_{\rm L,R}$ doublet and singlet Weyl spinors. 

Below the condensation scale $ \Lambda_{\rm HC}\sim 4\pi f$, the effective Lagrangian is given by
\begin{equation}\begin{aligned}
\mathcal{L}_{\rm  eff}&=\mathcal{L}_{\rm kin}-V_{\rm eff}.
\label{eq:total effective Lagrangian}
\end{aligned} \end{equation} 
%
The kinetic part of the Lagrangian is given by \begin{equation}\begin{aligned}
\label{eq:kinLag}
\mathcal{L}_{\mathrm{kin}}=\frac{f^2}{8}  \text{Tr} [D_{\mu}\Sigma_L^{\dagger}D^{\mu}\Sigma_L]+\frac{f^2}{8}  \text{Tr} [D_{\mu}\Sigma_R^{\dagger}D^{\mu}\Sigma_R].
\end{aligned} \end{equation} with \begin{equation}\begin{aligned} 
&D_\mu\Sigma_{L/R}=\partial_\mu \Sigma_{L/R}-i(G_{L/R,\mu}\Sigma_{L/R}+\Sigma_{L/R}G_{L/R,\mu}^T), \\
& G_{L/R,\mu}=g_{\rm L/R}W_{{\rm L/R},\mu}^i T_{\rm L/R}^i +g_{\rm Y'}B_\mu' T_{L{\rm Y'}/R{\rm Y'}}^3,  \nonumber
\end{aligned} \end{equation} where $ g_{\rm L,R,Y'} $ are the gauge couplings of $ \SU(2)_{\rm L} $, $ \SU(2)_{\rm R} $ and $ \UU(1)_{\rm Y'} $, respectively. Here the hypercharge coupling is given by $ g_{\rm Y}^{-2}=g_{\rm Y'}^{-2}+g_{\rm R}^{-2} $. Henceforth, the minimal value $g_{\rm R}$ can acquire is $g_{\rm R}^{\rm min} = g_{\rm Y}$.

At leading order, each source of symmetry breaking contributes independently to the effective potential in Eq.~(\ref{eq:total effective Lagrangian}): \begin{align} 
V_{\rm eff}\supset V_{\rm gauge}+V_{\rm top}+V_{\rm m}+V_{\rm B}.
\end{align} Here the EW gauge interactions in Eq.~(\ref{eq:kinLag}) yield the gauge loop contributions to the potential $ V_{\rm eff} $: %{\setlength{\thickmuskip}{.1\thickmuskip}
%\setlength{\medmuskip}{.1\medmuskip} 
\begin{equation}
\begin{aligned}
V_{\text{gauge}}= &-C_L f^4 \left\{ g_{\rm L}^2 \sum_i \text{Tr}\left[ T^i_{L{\rm L}}\Sigma_L (T^i_{L{\rm L}}\Sigma_L)^*\right] + g_{\rm Y'}^2  \text{Tr}\left[ T_{L{\rm Y'}}^3\Sigma_L (T_{L{\rm Y'}}^3\Sigma_L)^*\right] \right\} \\
&+ C_R f^4 \left\{ g_{\rm R}^2 \sum_i \text{Tr}\left[ T^i_{R{\rm R}}\Sigma_R (T^i_{R{\rm R}}\Sigma_R)^*\right]+ g_{\rm Y'}^2 \text{Tr}\left[ T_{R{\rm Y'}}^3\Sigma_L (T_{R{\rm Y'}}^3\Sigma_L)^*\right] \right\},
\end{aligned}\label{Gauge loop contribution (full)}
\end{equation}%}
where $ C_{L,R} $ encode non-perturbative low energy constants. The top loop contributions arising from the six-fermion operator
\begin{align} \label{eq:topmass supplementary}
\frac{\xi_t}{\Lambda_t^5} (Q_L^T P_L Q_L)(Q_R^T P_R Q_R) q_{{\rm L},3} q_{{\rm R},3}  + {\rm h.c.}
\end{align}	
yield the effective potential contribution:\begin{equation}\begin{aligned}
V_{\rm top}&=-\frac{1}{4}C_t y_t^2 f^4  \Big\{ \left|\Tr[P_L^1\Sigma_L]\right|^2 \left|\Tr[P_R^2\Sigma_R]\right|^2 \\ &+ \Tr[P_L^1\Sigma_L] \Tr[P_R^2\Sigma_R]\Tr[P_L^2\Sigma_L^\dagger] \Tr[P_R^1\Sigma_R^\dagger] \\& +(\text{L}\leftrightarrow \text{R})\Big\},
\end{aligned}
\end{equation} where $ C_t $ is a non-perturbative coefficient for the top loop, $ y_t $ (proportional to $ (\Lambda_{\rm HC}/\Lambda_t)^5 \xi_t  $) is identified by the top Yukawa coupling and the projectors, 
\begin{equation}\begin{aligned}
&(P_{L,R}^1)_{ij}=\frac{1}{2}(\delta_{1i}\delta_{3j}\pm\delta_{3i}\delta_{1j}), \qquad  (P_{L,R}^2)_{ij}=\frac{1}{2}(\delta_{2i}\delta_{4j}\pm\delta_{4i}\delta_{2j}),
\end{aligned}
\end{equation} select the components of $ Q_{L,R}^T Q_{L,R} $ that transform as doublets of $ \SU(2)_{\rm L,R} $. Moreover, the explicit hyper-fermion bilinear mass terms yield potential contributions:
\begin{align}
V_{\rm m} = 2\pi Z_L  \Tr[M_L \Sigma_L^\dagger ]+\rm h.c., \label{Effective mass Lagrangian VL and Dirac masses}
%\\
%V_{\rm B}&=C_B f^4  \Tr[B\Sigma_{R}^{\dagger}B\Sigma_{R}],
%\label{Effective mass Lagrangian}
\end{align} where $ M_L = {\rm diag}(m_{1}\epsilon,-m_{2}\epsilon) $ is the mass matrix of the $\mathbb{S}_L$ hyper-fermions. Finally, it is relevant to consider possible four-hyper-fermion operators in the $\mathbb{S}_R$ sector of the form $ Q_R Q_R Q_R Q_R $ 
%similar to the ETC term in Eq.~(26) in~\cite{Foadi:2007ue} 
which yield potential contributions~\cite{Foadi:2007ue}:
\begin{align}
V_{\rm B}&=C_B g_B^2 f^4  \Tr[B\Sigma_{R}^{\dagger}B\Sigma_{R}].
\label{Effective mass Lagrangian}
\end{align} The coefficients $ C_{L,R} $, $ C_{t} $, $ Z_L $ and $ C_B $ in Eq.~(\ref{Gauge loop contribution (full)})-(\ref{Effective mass Lagrangian}) are $ \mathcal{O}(1) $ form factors that can be computed on the lattice~\cite{Arthur:2016ozw}.
%
At leading order, the effective potential for the misalignment angle is given by
\begin{equation}
\begin{aligned} 
V_{\rm eff}^0=&-8\pi f^3 Z_L m_{UD} c_{\theta_L}- f^4 C_L  \widetilde{g}_L^2c_{\theta_L}^2 -f^4 C_t y_t^2 s_{\theta_L}^2  ,
\end{aligned} 
\end{equation} where $ m_{UD}\equiv m_1+m_2 $ and $  \widetilde{g}_L^2\equiv (3 g_{\rm L}^2 +g_{\rm Y'}^2)/2 $. By minimizing the above potential, $ \partial_{\theta_L} V_{\rm eff}^0=0 $, we obtain \begin{equation}\begin{aligned}
&c_{\theta_L} =\frac{4\pi Z_L m_{UD}}{f(C_t y_t^2- C_L\widetilde{g}_L^2)},  
\end{aligned}\end{equation} where the $ G_L/H_L $ part of the vacuum is aligned in a composite Higgs direction ($ 0<c_{\theta_L}<1 $), while the $ G_R/H_R $ part of the vacuum remains in a TC direction. The conditions for this vacuum alignment to be a stable minimum in the presence of these terms are $ \partial_{\theta_L\theta_L}V_{\rm eff}^0>0 $ and that all the squared masses of the pNGBs are positive. However, the condition $ \partial_{\theta_L\theta_L}V_{\rm eff}^0>0 $ is fulfilled by requiring $ m_h^2>0 $ due to the fact that $ \partial_{\theta_L\theta_L}V_{\rm eff}^0 = f^2 m_h^2  $. Therefore, we need that all the pNGBs have positive squared masses. The Higgs and $ \eta $ masses are \begin{equation}\begin{aligned}
&m_h^2 =2(C_t y_t^2 - C_L \widetilde{g}_L^2 )v_{\rm EW}^2,\quad \quad m_\eta^2 = m_h^2 /s_{\theta_L}^2,
\end{aligned}\end{equation} while the masses of the complex isotriplet composite scalars, $ \Pi_{CS,\overline{CS}}^0,\Pi^\pm_{CC},\Pi_{SS}^\pm $, in the $ \mathbb{S}_R $ sector are  \begin{equation}\label{eq:massesDM}\begin{aligned}
&m_{\Pi_{CS}^0}^2 = 2( C_Bg_B^2  - C_R \widetilde{g}_R^2 + C_t y_t^2 s_{\theta_L}^2)f^2, \\ 
&m_{\Pi_{CC}^\pm}^2=m_{\Pi_{SS}^\pm}^2 = m_{\Pi_{CS}^0}^2+2C_R g_{Y'}^2 f^2,
\end{aligned}\end{equation} where $  \widetilde{g}_R^2\equiv (-g_{\rm R}^2+g_{\rm Y'}^2)/2 $. To obtain a stable vacuum, we therefore need $ m_h^2 >0 $ and $ m_{\Pi_{CS}^0}^2>0 $. 
Following the common lore that the top loops tend to break the electroweak symmetry while gauge loops preserve it, we assume that the form factors $C_{L,R,t} > 0$. Hence, the masses squared are always positive, as long as the top loops dominate, as expected as the Yukawa coupling is larger than the gauge ones. Furthermore, in the $R$-coset, we find that $\widetilde{g}_R^2 \geq 0$ for $g_{\rm R} \geq \sqrt{2} g_{\rm Y}$, while it becomes positive for $g_{\rm Y} < g_{\rm R} < \sqrt{2} g_{\rm Y}$.   In the latter range, it tends to cancel the contribution of the top. As $m_{\Pi_{CS}}^0 = m_{DM}$, the magnitude of the Dark Matter candidate mass crucially depends on the value of these coefficients. In general, the first Eq.~\eqref{eq:massesDM} implies that the DM mass is of the order of the pNGB decays constants, i.e. $m_{DM} \sim f$. Small masses, of the order of GeV, could be obtained if a tuned cancellation is enacted. This could happen if the gauge contribution is large and positive, for $g_{\rm R} \gtrsim g_{\rm Y}$, or for $C_B < 0$.

As discussed in the main text, for light DM mass the annihilation is dominantly into the light pNGB associated to the $\UU(1)_\Theta$ symmetry. If either of the vector-like masses $ m_1 $ or $m_2$ are vanishing, the pNGB $ \Theta $ state mixes with the $ \mathbb{S}_L $ pNGB $ \eta $ state, resulting in that the mass eigenstate $ \widetilde{\Theta} $, consisting mostly of $ \Theta $, is massless while $ \widetilde{\eta} $ has a mass of order $ f $:\begin{equation}\begin{aligned}
&m_{\widetilde{\Theta}}^2=0,\quad \quad m_{\widetilde{\eta}}^2=\frac{1}{4} \frac{m_h^2}{s_{\theta_L}^2} (5+c_{2\theta_L})\approx  \frac{3m_h^2}{2s_{\theta_L}^2}.
\end{aligned}\end{equation} However, the $ \widetilde{\Theta} $ state can achieve a small mass from its mixing with a $ \Theta' $ state corresponding to the $ \UU(1)$ symmetry which is quantum anomalous. In addition, the mass of $ \Theta' $ is generated by instanton effects related to the $ \UU(1) $ anomaly~\cite{Belyaev:2016ftv}. 

Thus, for DM masses below the $W_{\rm R}$ mass, the dominant annihilation channel is $ \Pi_{X} \overline{\Pi}_{X} \to \widetilde{\Theta}\widetilde{\Theta}$ with the coupling $ \lambda_{XX \widetilde{\Theta} \widetilde{\Theta}} $ given by\begin{equation}\begin{aligned}
&\mathcal{L}_{\rm eff}\supset \lambda_{XX\widetilde{\Theta}\widetilde{\Theta}}\Pi_{CS}^0\Pi_{\overline{CS}}^0\widetilde{\Theta}\widetilde{\Theta}
\end{aligned}\end{equation} with \begin{equation}\begin{aligned}
\lambda_{XX\widetilde{\Theta}\widetilde{\Theta}}=&4C_t y_t^2 s_{\theta_L}^2 \frac{c_{\theta_L}}{\sqrt{2+c_{\theta_L}^2}}\approx \frac{4}{\sqrt{3}}C_t y_t^2 \left(\frac{v_{\rm EW}}{f}\right)^2 \equiv \lambda_0  \left(\frac{v_{\rm EW}}{f}\right)^2.  \nonumber
\end{aligned}\end{equation} 
This implies that $\lambda_0 \sim \frac{4}{\sqrt{3}}C_t y_t^2$, which could be an order 1 number.\\


In the scenario with $ \mathcal{R}_R = F $ (fundamental, pseudo-real) of $ G_{\rm HC}=\SP(2N_{\rm HC}) $, the DM candidate is identified by a complex isosinglet, $ \Pi_{CS,\overline{CS}} $, where its mass is given by \begin{equation}\begin{aligned}
&m_{\Pi_{CS}}^2 = 2( C_Bg_B^2  - C_R \widetilde{g}_R^2 + C_t y_t^2 s_{\theta_L}^2)f^2,
\end{aligned}\end{equation} where $ \widetilde{g}_R^2=(3g_{\rm R}^2+g_{\rm Y'}^2)/2 $ which is always positive. Due to the fact that $ s_{\theta_L}\ll 1 $, $ m_{\Pi_{CS}}^2 $ is negative when $ C_B g_B^2=0 $ and therefore a small DM mass, $ m_{\Pi_{CS}}\ll f $, can be achieved by tuning $ C_B g_B^2 $ to a certain value of order unity. Furthermore, in the scenarios with the top mass arising from PC operators, the DM mass can also be tuned by the term $ C_B g_B^2 $ to small values in both scenarios.  These models are inspired by the work in Ref.~\cite{Ferretti:2013kya}.




%\begin{equation}\begin{aligned}
%\lambda_{XX\widetilde{\Theta}\widetilde{\Theta}}=&4C_t y_t^2 \left(\frac{v_{\rm EW}}{f_L}\right)^2 \frac{c_{\theta_L}}{\sqrt{2+c_{\theta_L}^2}}\approx \frac{4}{\sqrt{3}}C_t y_t^2 \left(\frac{v_{\rm EW}}{f_L}\right)^2 \\
%\lambda_{XX\widetilde{\eta}\widetilde{\eta}}=&\frac{\sqrt{2}}{c_{\theta_L}}\lambda_{XX\widetilde{\Theta}\widetilde{\Theta}}\approx \sqrt{2}\lambda_{XX\widetilde{\Theta}\widetilde{\Theta}}. \nonumber
%\end{aligned}\end{equation} 


%----------------------------------------------------------------------
%\clearpage
\section{Examples of theories featuring the Techni-Composite Higgs mechanism}

In the main body of the article, we studied in detail one specific model based on a gauge symmetry $\SP(2N)_{\rm HC}$ and with fermions in two different representations. However, the same mechanism can be found in many other models, with different possibilities for the $ L $ and $ R $-cosets, as listed in Tables~\ref{table:Lcosets} and~\ref{table:Rcosets}, respectively.  Here we list the quantum numbers of the HC fermions needed to obtain the minimal cosets, for the three classes of HC representations: pseudo-real, real and complex.


\begin{table}[htb]
	\centering
	\begin{tabular}{cccccc}
		\hline
		&$G_{\rm HC}$		&$\SU(2)_{\rm L}$	&$\SU(2)_{\rm R}$	&$ \UU(1)_{\rm Y'} $	&$\UU(1)_{TB,L}$\\
		\hline
		\multicolumn{6}{c}{pseudo-real} \\ \hline
		$ (U,D) $	&$\mathcal{R}_{L}$				&$ \Box $		&1			&0				& 0\\
		$ \widetilde{U} $	&$\mathcal{R}_{L}$					&1			&1			&$ -1/2	 $		& 0	\\
		$ \widetilde{D} $	&$\mathcal{R}_{L}$				&1			&1			&$ +1/2 $			& 0	\\
		\hline
		\multicolumn{6}{c}{complex} \\ \hline
		$ (U,D) $	&$\mathcal{R}_{L}$				&$ \Box $		&1			&0				& 1\\
		$ \widetilde{U} $	&$\mathcal{R}_{L}$					&1			&1			&$ -1/2	 $		& 1	\\
		$ \widetilde{D} $	&$\mathcal{R}_{L}$				&1			&1			&$ +1/2 $			& 1	\\
		$ (U^c,D^c) $	&$\mathcal{R}_{L}^\ast$				&$ \Box $		&1			&0				& -1\\
		$ \widetilde{U}^c $	&$\mathcal{R}_{L}^\ast$					&1			&1			&$ +1/2	 $		& -1	\\
		$ \widetilde{D}^c $	&$\mathcal{R}_{L}^\ast$				&1			&1			&$ -1/2 $			& -1	\\
		
		\hline
		\multicolumn{6}{c}{real} \\ \hline
		$ (U,D) $	&$\mathcal{R}_{L}$				&$ \Box $		&1			&1/2				& 0\\
		$ (\widetilde{U},\widetilde{D}) $	&$\mathcal{R}_{L}$		&$ \Box $		&1			&-1/2				& 0\\
		$ X $	&$\mathcal{R}_{L}$					&1			&1			& 0			& 0	\\ \hline
	\end{tabular}
	\caption{Fermion field content and their charges for the minimal L-cosets.}
	\label{table:Lcosets}
\end{table}


\begin{table}[htb]
	\centering
	\begin{tabular}{ccccccc}
		\hline
		&$G_{\rm HC}$		&$\SU(2)_{\rm L}$	&$\SU(2)_{\rm R}$	&$ \UU(1)_{\rm Y'} $	&$\UU(1)_X$ & $\UU(1)_{TB,R}$\\
		\hline
		\multicolumn{7}{c}{pseudo-real} \\ \hline
		$ (C,S) $	&$\mathcal{R}_{R}$						&1			&$ \Box $		&0				&$ +1$	& 0\\
		$ \widetilde{C} $	&$\mathcal{R}_{R}$					&1			&1			&$ -1/2 $			&$ -1$ & 0\\
		$ \widetilde{S} $	&$\mathcal{R}_{R}$					&1			&1			&$ +1/2 $			&$ -1$& 0\\		\hline
		\multicolumn{7}{c}{complex} \\ \hline
		$ (C,S) $	&$\mathcal{R}_{R}$						&1			&$ \Box $		&0				&$ +1$	& 1\\
		$ \widetilde{C} $	&$\mathcal{R}_{R}^\ast$					&1			&1			&$ -1/2 $			&$ -1$ & $-1$\\
		$ \widetilde{S} $	&$\mathcal{R}_{R}^\ast$					&1			&1			&$ +1/2 $			&$ -1$ & $-1$\\		\hline
		\multicolumn{7}{c}{real} \\ \hline
		$ (C,S) $	&$\mathcal{R}_{R}$						&1			&$ \Box $		&0				&$ +1$ & 0	\\
		$ \widetilde{C} $	&$\mathcal{R}_{R}$					&1			&1			&$ -1/2 $			&$ -1$ & 0\\
		$ \widetilde{S} $	&$\mathcal{R}_{R}$					&1			&1			&$ +1/2 $			&$ -1$ & 0\\ \hline
	\end{tabular}
	\caption{Fermion field content and their charges for the minimal R-cosets.}
	\label{table:Rcosets}
\end{table}


Finally, in Table~\ref{tab:examples} we provided some examples of gauge-fermion theories generating various combinations for the $L$ and $R$-cosets. In the cases with $\mathcal{R}_L = \mathcal{R}_R$, the global symmetry is extended to a single simple group that contains the $L$ and $R$ sub-cosets


%\begin{widetext}
\begin{table}[htb]
	\centering
	\begin{tabular}{|l|c|c|c|c|l|}
		\hline
		$G_{\rm HC}$ & $\mathcal{R}_L$ & dim($\mathcal{R}_L$) & $\mathcal{R}_R$ & dim($\mathcal{R}_R$) & Annotations\\ \hline 
		\multicolumn{6}{c}{\phantom{\Big(} $\SU(4)/ \SP(4)_L \otimes \SU(4)/\SO(4)_R \otimes \UU(1)_\Theta/\varnothing$} \\ \hline
		$\SP(2N)_{\rm HC}$ & $F$ & $2N$ & $A$ & $N (2N-1)-1$ & $N$ odd to avoid Witten anomalies \\
		$\SP(2N)_{\rm HC}$ & $F$ & $2N$ & $Adj$ & $N (2N+1)$ & $N$ even to avoid Witten anomalies \\
		\hline
		\multicolumn{6}{c}{\phantom{\Big(} $\SU(4)^2/\SU(4)_L \otimes \SU(4)/\SO(4)_R \otimes \UU(1)_\Theta/\varnothing \otimes \UU(1)_{TB, L}$} \\ \hline
		$\SU(4)_{\rm HC}$ & $F$ & $4$ & $A_2$ & $6$ & - \\
		$\SO(10)_{\rm HC}$ & $Spin$ & $16$ & $F$ & $10$ & - \\
		\hline
		\multicolumn{6}{c}{\phantom{\Big(} $\SU(4)^2/\SU(4)_L \otimes \SU(2)^2/\SU(2)_R \otimes \UU(1)_\Theta/\varnothing \otimes \UU(1)_{TB,L} \otimes \UU(1)_{TB,R}$} \\ \hline
		$\SU(5)_{\rm HC}$ & $F$ & $5$ & $A_2$ & $10$ & - \\
		\hline
		\multicolumn{6}{c}{\phantom{\Big(} $\SU(5)/\SO(5)_L \otimes \SU(4)/\SO(4)_R \otimes \UU(1)_\Theta/\varnothing$} \\ \hline
		$\SO(7)_{\rm HC}$ & $F$ & $7$ & $Spin$ & $8$ & - \\
		\hline
		\multicolumn{6}{c}{\phantom{\Big(} $\SU(5)/\SO(5)_L \otimes \SU(4)/\SP(4)_R \otimes \UU(1)_\Theta/\varnothing$} \\ \hline
		$\SP(2N)_{\rm HC}$ & $A$ & $N (2N-1)-1$ & $F$ & $2N$ & $N \geq 2$ \\
		\hline
		\multicolumn{6}{c}{\phantom{\Big(} $\SU(5)/\SO(5)_L \otimes \SU(2)^2/\SU(2)_R \otimes \UU(1)_\Theta/\varnothing \otimes \UU(1)_{TB,R}$} \\ \hline
		$\SU(4)_{\rm HC}$ & $A$ & $6$ & $F$ & $4$ & - \\
		$\SO(10)_{\rm HC}$ & $F$ & $10$ & $Spin$ & $16$ & - \\
		\hline
		\multicolumn{6}{c}{\phantom{\Big(} $\SU(8)/\SP(8)$} \\ \hline
		$\SP(2N)_{\rm HC}$ & $F$ & $2N$ & $F$ & $2N$ & - \\
		\hline
		\multicolumn{6}{c}{\phantom{\Big(} $\SU(9)/\SO(9)$} \\ \hline
		$\SU(4)_{\rm HC}$ & $A$ & $6$ & $A$ & $6$ & - \\
		$\SO(10)_{\rm HC}$ & $F$ & $10$ & $F$ & $10$ & - \\
		\hline
		\multicolumn{6}{c}{\phantom{\Big(} $\SU(6)^2/\SU(6) \otimes \UU(1)_{TB}$} \\ \hline
		$\SU(N)_{\rm HC}$ & $F$ & $N$ & $F$ & $N$ & - \\
		$\SU(5)_{\rm HC}$ & $A$ & $10$ & $A$ & $10$ & - \\
		\hline
	\end{tabular}
	\caption{\label{tab:examples} Examples of gauge fermion theories leading to the Techni-Composite Higgs models.}
\end{table}
%\end{widetext}


%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\section{Asymmetry sharing}
We here in detail show  how the asymmetric dark matter relic can be calculated \cite{Harvey:1990qw,Ryttov:2008xe}.
First, note that at high temperatures the particle number density $ n_+ $ and the anti-particle number density $ n_- $ of a given species are given by
\begin{align}
n_\pm =  g \int \frac{d^3k}{(2\pi)^3}\frac{g}{e^{(E\mp\mu)\beta}-\eta} \qq{with} \begin{aligned}
\eta &= +1 \text{ for bosons} \\[-1ex]
\eta &= -1 \text{ for fermions}
\end{aligned}
\end{align}
where $ g $ is the number of internal degrees of freedom, $ \mu $ is the chemical potential of the particle species and $ \beta = 1/T$ (with $ k_B = 1 $). 
At the freeze-out temperature of sphalerons, $ T_F $, we have $ \mu/T_F\ll 1$ such that the difference in particle numbers of a given species is given by
\begin{gather}
n = n_+ - n_- = gT_F^3 \frac{\mu}{T_F}\frac{\sigma(m/T_F)}{6}, \label{eq:assymetric number density}
\end{gather}
which reveals that the chemical potentials are the relevant quantities.
Here the statistical suppression factor $ \sigma $ is
\begin{gather}
\sigma(m/T_F)=\begin{cases}
\frac{6}{4\pi^2}\int_{0}^{\infty} dx x^2 \cosh[-2](\frac{1}{2}\sqrt{x^2+(m/T_F)^2})	&\text{for fermions}\\
\frac{6}{4\pi^2}\int_{0}^{\infty} dx x^2 \sinh[-2](\frac{1}{2}\sqrt{x^2+(m/T_F)^2})	&\text{for bosons.}
\end{cases} 
%\text{for fermions (top) and bosons (bottom).}
\label{Eq:statfunc}
\end{gather}
The statistical factor $ \sigma(m/T_F) $ is normalized such that
\begin{gather}
\lim_{m/T_F\to 0} \sigma(m/T_F) = \begin{cases}
1 &\text{for fermions,} \\
2 &\text{for bosons,}
\end{cases} 
\end{gather}
while $\sigma(m/T_F)\simeq2 (m/2\pi T_F)^{3/2} e^{-m/T_F}$ for large $m/T_F\gg 1$. 
In therms of chemical potentials, the ratio of DM and baryon energy densities can be expressed as
\begin{gather}
\frac{\Omega_{DM}}{\Omega_B} = \frac{\frac{1}{2}m_{DM} }{m_P}\left|\frac{\mu_{X}}{\mu_B}\right|\sigma\left(\frac{m_{DM}}{2 T_F}\right),
\end{gather}
where we neglected the $ \sigma(m / 2 T_F) $ for the SM fermions. The task is then to calculate the total chemical potential $ \mu_{X} $ of all fermions charged under $\UU(1)_X$  and the total chemical potential of all baryons $ \mu_B $

%Since the baryon, lepton and technibaryon numbers $ B $, $ L $ and $ TB $ are proportional to the number densities we can express them purely in terms of chemical potentials and the relevant statistical suppression factors. 

To study the chemical potentials we adopt the we adopt the notation of Ryttov-Sannino \cite{Ryttov:2008xe} and Harvey-Turner \cite{Harvey:1990qw}. The equilibrium condition from sphalerons, as written in this convention, was already given in the main text. Additionally, the 6-fermion operators, given by Eq.~\eqref{eq:topmass supplementary}, lead to equilibrium conditions of the form
\begin{align}
\begin{aligned}
\mu_{UL}-\mu_{UR}+\mu_{SR}-\mu_{SL}		-\mu_{u{\rm L},i}+\mu_{u{\rm R},i} 		&=0,\\
\mu_{UL}-\mu_{UR}+\mu_{SR}-\mu_{SL}		+\mu_{d{\rm L},i}-\mu_{d{\rm R},i} 		&=0,\\
\mu_{UL}-\mu_{UR}+\mu_{SR}-\mu_{SL}		-\mu_{\nu {\rm L},i}+\mu_{\nu{\rm R},i}&=0,\\
\mu_{UL}-\mu_{UR}+\mu_{SR}-\mu_{SL}		+\mu_{e{\rm L},i}-\mu_{e{\rm R},i} 		&=0,
\end{aligned}\label{eq:6-fermion block 1}
\end{align}
and
\begin{align}
\begin{aligned}
\mu_{DL}-\mu_{DR}+\mu_{CR}-\mu_{CL}		-\mu_{u{\rm R},i}+\mu_{u{\rm L},i}		&=0,\\
\mu_{DL}-\mu_{DR}+\mu_{CR}-\mu_{CL}		+\mu_{d{\rm R},i}-\mu_{d{\rm L},i}		&=0,\\
\mu_{DL}-\mu_{DR}+\mu_{CR}-\mu_{CL}		-\mu_{\nu{\rm R},i}+\mu_{\nu{\rm L},i}&=0,\\
\mu_{DL}-\mu_{DR}+\mu_{CR}-\mu_{CL}		+\mu_{e{\rm R},i}-\mu_{e{\rm L},i}		&=0,\\
\end{aligned}\label{eq:6-fermion block 2}
\end{align}
where the index $ _i $ refers to the three generations of SM fermions, each of which has equilibrium conditions of this form. However, depending on the temperature, only some generations of quarks and leptons have efficient 6-fermion operators. As was pointed out in the letter, a fermion $\psi$, receiving its mass $m_\psi$ from such an interaction is in equilibrium at a temperature $ T $ if~\cite{Davidson:2008bu, Deppisch:2017ecm}
\begin{gather}
2.3\times 10^4\times \sqrt{\frac{10\text{ TeV}}{f}}\frac{m_\psi}{v_{\rm EW}} \gtrsim \left(\frac{f}{T}\right)^{9/2}. \label{eq:in equilibrium condition}
\end{gather}
We assume that the conditions corresponding to \eqref{eq:6-fermion block 1} and \eqref{eq:6-fermion block 2} apply for any fermions for which the condition \eqref{eq:in equilibrium condition} is satisfied for all participating species at the condensation temperature $ T=f $.

Furthermore, thermal equilibrium in the electroweak interactions imply the following conditions:
\begin{align}
\begin{aligned}\label{EW interactions equilibrium equations}
\mu_{u{\rm L},i}&=\mu_{d{\rm L},i}+\mu_{W\rm L}, & \mu_{u{\rm R},i}&=\mu_{d{\rm R},i}+\mu_{W\rm R}, \\
\mu_{e{\rm L},i}&=\mu_{\nu{\rm L}, i}+\mu_{W\rm L}, & \mu_{e{\rm R},i}&=\mu_{\nu{\rm R}, i}+\mu_{W\rm R}, \\ 
\mu_{DL}&=\mu_{UL}+\mu_{W\rm L}, & \mu_{SL}&=\mu_{CL}+\mu_{W\rm R}. \\ 
\end{aligned}
\end{align}
The equilibrium is constrained by conditions on the net charge of plasma. To quantify this, consider the eigenvalues of third the components of the isospins of $ \SU(2)_{\rm L,R} $, which are
\begin{align}
T_{L\rm L}^3 = &3\times \sum_i\left( \frac{1}{2}\mu_{u{\rm L},i}-\frac{1}{2}\mu_{d{\rm L},i}\right) + \sum_i\left( \frac{1}{2}\mu_{\nu{\rm L}, i}-\frac{1}{2}\mu_{e{\rm L}, i} \right)-4\mu_{W\rm L}+2\left( \frac{1}{2}\mu_{UL}-\frac{1}{2}\mu_{DL} \right),\\
T_{R\rm R}^3 = &3\times \sum_i\left( \frac{1}{2}\mu_{u{\rm R},i}-\frac{1}{2}\mu_{d{\rm R},i}\right) + \sum_i\left( \frac{1}{2}\mu_{\nu{\rm R}, i}-\frac{1}{2}\mu_{e{\rm R}, i} \right)-4\mu_{W\rm R}+2\left( \frac{1}{2}\mu_{CR}-\frac{1}{2}\mu_{SR} \right).
\end{align}
The overall electric charge, $ Q = T_{L\rm L}^3+T_{R\rm R}^3+Y' $, is then
\begin{align}
Q = &3\times \sum_i\left( \frac{2}{3}\mu_{u{\rm L},i}+\frac{2}{3}\mu_{u{\rm R},i}-\frac{1}{3}\mu_{d{\rm L},i}-\frac{1}{3}\mu_{d{\rm R},i} \right)+\sum_i\left( -1 \mu_{e{\rm L},i}-1 \mu_{e{\rm R},i}+0\mu_{\nu{\rm  L}, i}+0\mu_{\nu{\rm  R}, i} \right)\notag\\
&+ d(\mathcal{R}_L)\left( \frac{1}{2}\mu_{UL}+\frac{1}{2}\mu_{UR}-\frac{1}{2}\mu_{DL}-\frac{1}{2}\mu_{DR} \right) + d(\mathcal{R}_R)\left( \frac{1}{2}\mu_{CL}+\frac{1}{2}\mu_{CR}-\frac{1}{2}\mu_{SL}-\frac{1}{2}\mu_{SR} \right)\\ 
%& +\frac{1}{2}(\mu_{NL}-\mu_{EL}+\mu_{NR}-\mu_{ER})\notag\\
&-4\mu_{W\rm L}-4\mu_{W\rm R}. \notag
\end{align} 
The conditions imposed depend on the type of phase transition. Above the transition, where $ \SU(2)_{\rm L,R} $ are good symmetries, $ T_{ {L\rm L},{R\rm R}}^3 $ must vanish. If the phase transition is sudden, i.e. first order, then this property is assumed to be inherited by the relic such that relevant condition is
\begin{gather}
Q = 0, \quad T_{L \rm L}^3 = 0, \quad T_{R \rm R}^3 = 0.\label{First-order condition,app}
\end{gather}
Below the transition, $ \SU(2)_{\rm L,R} $ are broken, such that $ T_{{L\rm L},{R\rm R}}^3 $ need no longer vanish. If the phase transition is gradual, i.e. second order, then this leads to violation of $ T_{{L\rm L},{R\rm R}}^3 $ conditions. Instead, the VEV drives the chemical potentials of neutral condensates to zero, such that the relevant condition is 
\begin{gather}
\begin{gathered}
Q = 0, \quad \mu_{UL}-\mu_{UR}= 0, \quad \mu_{CR}-\mu_{CL}= 0. \label{Second-order condition,app}
\end{gathered}
\end{gather}
We are ultimately interested in comparing the total baryon and DM densities, which depend on the total chemical potentials of the baryons and technibaryons (charged under $\UU(1)_X$), which are
\begin{align} \label{Baryon,lepton, TB number}
\mu_B &= \sum_i \left(\mu_{u{\rm L},i}+\mu_{u{\rm R},i} +\mu_{d{\rm L},i}, + \mu_{d{\rm R},i} \right), \\
%\mu_L = \sum_i \left( \mu_{\nu L, i}+\mu_{\nu R, i}+\mu_{eL, i}+\mu_{eR, i} \right), \\
\mu_{X} &= d(\mathcal{R}_R) \left( \mu_{CR}+\mu_{CL}+\mu_{SL}+\mu_{SR} \right).%\sigma(m_{TB}/T_F)
\end{align}
%where $ m_{TB} $ is the effective mass of the $ \mathbb{S}_R $ fermions and the $ N_R $ is dimension of the representation $ \mathcal{R}_2 $ under $ G_{\rm HC} $ for the right-handed sector ($ N_R=2 $ or $ N_R=3 $ for the fundamental or adjoint representation when $ G_{\rm HC}=\SU(2)_{\rm HC} $, respectively). %We give the expressions for the charges in the appendix. 
Solving all the above conditions for $ \mu_{X} $ and $ \mu_{B} $ we find
\begin{gather}
\left|\frac{\mu_{X}}{\mu_B}\right| = 2\left(3+\frac{L}{B}\right), \label{eq:mu ratio}
\end{gather}
if 6-fermion operations are inefficient for at least one generation but efficient for at least one other generation. Since the occupation numbers are proportional to the chemical potentials, we can identify $ \left|\mu_{X}/\mu_B\right| = \left|X/B\right| $. If all generations are in equilibrium, then the lepton number is constrained to $ L=-3B $ so that $ \mu_{X}=0 $. Furthermore, if 6-fermion operators are inefficient for all generations, then $ \mu_{X} $ is unconstrained in the case of first-order transitions while Eq. \eqref{eq:mu ratio} applies for the case of second-order transitions.




%When the right-handed sector is in the adjoint representation with fermion content as in Table~\ref{table:fullmodelvar}, then the overall electric charge, where $ Q = T_{\rm L}^3+T_{\rm R}^3+Y' $, is 
%\begin{align*}
%\begin{aligned}
%Q = &3\times 3\left( \frac{2}{3}\mu_{uL,i}+\frac{2}{3}\mu_{uR,i}-\frac{1}{3}\mu_{dL,i}-\frac{1}{3}\mu_{dR,i} \right)
%+\sum_i\left( -1 \mu_{eL,i}-1 \mu_{eR,i}+0\mu_{\nu L, i}+0\mu_{\nu R, i} \right)\\
%&+ 2\left( \frac{1}{2}\mu_{UL}+\frac{1}{2}\mu_{UR}-\frac{1}{2}\mu_{DL}-\frac{1}{2}\mu_{DR} \right) 
%+ 3\left( 0\mu_{CL}-1\mu_{CR}+0\mu_{SL}-1\mu_{SR} \right)\\ & -4\mu_{W\rm L}-4\mu_{W\rm R},
%\end{aligned}
%\end{align*} and the third components of the isospins of $ \SU(2)_{\rm L,R} $ are \begin{align*}
%\begin{aligned}
%T_{\rm L}^3 = &3\times 3\left( \frac{1}{2}\mu_{uL,i}-\frac{1}{2}\mu_{dL,i}\right) + \sum_i\left( \frac{1}{2}\mu_{\nu L, i}-\frac{1}{2}\mu_{eL, i} \right)-4\mu_{W\rm L}+2\left( \frac{1}{2}\mu_{UL}-\frac{1}{2}\mu_{DL} \right),\\
%T_{\rm R}^3 = &3\times 3\left( \frac{1}{2}\mu_{uR,i}-\frac{1}{2}\mu_{dR,i}\right) -4\mu_{W\rm R}+3\left( \frac{1}{2}\mu_{CR}-\frac{1}{2}\mu_{SR} \right).
%\end{aligned}
%\end{align*}
%
%When the $ \mathbb{S}_R $ sector is in the fundamental representation and $ G_{\rm HC}=\SU(2)_{\rm HC} $, the overall electric charge $ Q = T_{\rm L}^3+T_{\rm R}^3+Y' $ is
%\begin{align*}
%\begin{aligned}
%Q = &3\times 3\left( \frac{2}{3}\mu_{uL,i}+\frac{2}{3}\mu_{uR,i}-\frac{1}{3}\mu_{dL,i}-\frac{1}{3}\mu_{dR,i} \right)
%+\sum_i\left( -1 \mu_{eL,i}-1 \mu_{eR,i}+0\mu_{\nu L, i}+0\mu_{\nu R, i} \right)\\
%&+ 2\left( \frac{1}{2}\mu_{UL}+\frac{1}{2}\mu_{UR}-\frac{1}{2}\mu_{DL}-\frac{1}{2}\mu_{DR} \right) 
%+ 2\left( \frac{1}{2}\mu_{CL}+\frac{1}{2}\mu_{CR}-\frac{1}{2}\mu_{SL}-\frac{1}{2}\mu_{SR} \right)\\ & -4\mu_{W\rm L}-4\mu_{W\rm R},
%\end{aligned}
%\end{align*}
%and the third components of the isospins of $ \SU(2)_{\rm L,R} $ are
%\begin{gather*}
%\begin{gathered}
%T_{\rm L}^3 = 3\times 3\left( \frac{1}{2}\mu_{uL,i}-\frac{1}{2}\mu_{dL,i}\right) + \sum_i\left( \frac{1}{2}\mu_{\nu L, i}-\frac{1}{2}\mu_{eL, i} \right)-4\mu_{W\rm L}+2\left( \frac{1}{2}\mu_{UL}-\frac{1}{2}\mu_{DL} \right),\\
%T_{\rm R}^3 = 3\times 3\left( \frac{1}{2}\mu_{uR,i}-\frac{1}{2}\mu_{dR,i}\right) + \sum_i\left( \frac{1}{2}\mu_{\nu R, i}-\frac{1}{2}\mu_{eR, i} \right)-4\mu_{W\rm R}+2\left( \frac{1}{2}\mu_{CR}-\frac{1}{2}\mu_{SR} \right).
%\end{gathered}
%\end{gather*}


%\bibliographystyle{JHEP-2-2}

%\bibliography{RTC-LCH.bib}


\end{document}

